MixtureVitae: Open Web-Scale Pretraining Dataset With High Quality Instruction and Reasoning Data Built from Permissive-First Text Sources

We present MixtureVitae, an open-access pretraining corpus built to minimize legal risk while providing strong downstream performance. MixtureVitae follows a permissive-first, risk-mitigated sourcing strategy that combines public-domain and permissively licensed text (e.g., CC-BY/Apache) with carefully justified low-risk additions (e.g., government works and EU TDM-eligible sources). MixtureVitae adopts a simple, single-stage pretraining recipe that integrates a large proportion of permissive synthetic instruction and reasoning data-signals typically introduced during post-training and generally scarce in permissive web corpora. We categorize all sources into a three-tier scheme that reflects varying risk levels and provide shard-level provenance metadata to enable risk-aware usage. In controlled experiments using the open-sci-ref training protocol (fixed architectures and hyperparameters; 50B and 300B token budgets across 130M-1.7B parameters), models trained on MixtureVitae consistently outperform other permissive datasets across a suite of standard benchmarks, and at the 1.7B-parameters/300B-tokens setting, they surpass FineWeb-Edu and approach DCLM late in training. Performance is particularly strong on MMLU and on math and code benchmarks: a 1.7B model pretrained on 300B MixtureVitae tokens matches or exceeds a strong 1.7B instruction-tuned baseline on GSM8K, HumanEval, and MBPP, despite using over 36 times fewer tokens (300B vs. ~11T). Supported by a thorough decontamination analysis, these results show that permissive-first data with high instruction and reasoning density, tiered by licensing and provenance-related risk, can provide a practical and risk-mitigated foundation for training capable LLMs, reducing reliance on broad web scrapes without sacrificing competitiveness. Code: https://github.com/ontocord/mixturevitae

==> tables/breakdown_by_license_type.tex <==
% This code is compatible with your existing packages.
% Assumes you have already loaded: booktabs, longtable, hyperref
% \refstepcounter{table}
\begin{longtable}{p{4cm} p{7cm} r}

% This is the caption that will appear above the table.
% \caption{Breakdown of the Dataset by Source and License}
% \label{tab:breakdown_by_license_type}\\

% --- HEADERS ---
% This header appears on the FIRST page of the table.
\toprule
\textbf{License Type} & \textbf{Source / Data} & \textbf{Size} \\
\midrule
\endfirsthead

% This header appears on ALL SUBSEQUENT pages of the table.
\multicolumn{3}{c}%
{{\bfseries\tablename\ \thetable{} -- continued from previous page}} \\
\toprule
\textbf{License Type} & \textbf{Source / Data} & \textbf{Size} \\
\midrule
\endhead

% --- FOOTERS ---
% This footer appears at the bottom of every page EXCEPT the last one.
\bottomrule
\multicolumn{3}{r}{{Continued on next page}} \\
\endfoot

% This footer appears only on the LAST page of the table.
\bottomrule

\endlastfoot

% --- WEB SECTION ---
\multicolumn{3}{c}{\large\textbf{Web}} \\
\multicolumn{3}{l}{\footnotesize\textit{*All data in this section subject to Common Crawl Terms of Uses}} \\
\midrule
Public Domain (copyright expired) & US Federal governmental websites including a small portion of Project Gutenberg out of copyright literature inclded in the web portion, & 6B \\
\addlinespace % Adds a little vertical space for readability
Risk-mitigated government data & Non US federal government works & 11B \\
\addlinespace
CC-BY-SA* licenses or more permissive & Specific curated websites and heuristicly mathced websites (See Sec. J) & 2B \\
\midrule

% --- CURATED SECTION ---
\multicolumn{3}{c}{\large\textbf{Curated}} \\
\midrule
Public Domain & US Case law, SEC 10K, Europat, USPTO & 4 B \\
\addlinespace
CC-BY-SA* licenses or more permissive & News, wiki,  Youtube, peS2o, Pubmed, Arxiv, Stackexchange, elsevier-oa-cc-by,  & 24.67+10.31+5.21+3.69B \\
\addlinespace
Non-GPL open source license (e.g., Open-RAIL, Apache, MIT) & Stackv1 and its derivatives & 6.4+18.64 B \\
\midrule

% --- INSTRUCT SECTION ---
\multicolumn{3}{c}{\large\textbf{Instruct}} \\
\midrule
CC-BY.* licenses or more permissive & math\_word\_problems & 1.2 GB \\
& Nemo\_science\_math & 79 GB \\
\addlinespace
Non-GPL open source license (e.g., Apache, MIT) & Prism\_math (cc-by-4.0), Os-q2, Formatted\_text (only websights), misc\_instruct (cc-by-4.0) & 105 GB \\
& Glaiveai-reasoning (apache), Ring-lite (apache), Open\_thoughts (apache), Ling-coder (apache), Few-shot (from \href{https://huggingface.co/datasets/Muennighoff/P3}{P3}, apache), misc\_instruct (apache 2.0), Math (apache 2.0) & 458.6 GB \\
& dart-math, misc\_instruct (MIT) & 5 GB \\
& pyedu\_reasoning & 11 GB \\
% \captionof{table}{Breakdown of the Dataset by Source and License}
\end{longtable}
\addtocounter{table}{-1} % Corrects the counter for the caption command
\begin{center}
    \captionof{table}{Breakdown of the Dataset by Source and License}
    \label{tab:breakdown_by_license_type}
\end{center}

